Two-Face: Adversarial Audit of Commercial Face Recognition Systems

Computer vision applications like automated face detection are used for a variety of purposes ranging from unlocking smart devices to tracking potential persons of interest for surveillance. Audits of these applications have revealed that they tend to be biased against minority groups which result in unfair and concerning societal and political outcomes. Despite multiple studies over time, these biases have not been mitigated completely and have in fact increased for certain tasks like age prediction. While such systems are audited over benchmark datasets, it becomes necessary to evaluate their robustness for adversarial inputs. In this work, we perform an extensive adversarial audit on multiple systems and datasets, making a number of concerning observations - there has been a drop in accuracy for some tasks on CELEBSET dataset since a previous audit. While there still exists a bias in accuracy against individuals from minority groups for multiple datasets, a more worrying observation is that these biases tend to get exorbitantly pronounced with adversarial inputs toward the minority group. We conclude with a discussion on the broader societal impacts in light of these observations and a few suggestions on how to collectively deal with this issue.

==> experiment-backup.tex <==
\section{Experiments and Observations}
\label{sec:experiments}
%\todo{Informative captions needed for Figures and Tables.}
In this section, we present the experimental setup and the experiments conducted, followed by a discussion on the observations for the general audits and the adversarial audits conducted on the chosen datasets.
%of change in accuracy since previous audits, change in accuracy between original images and perturbed images and the dispartieis, if any, amongst the different intersectional groups within each dataset.

\subsection{Tasks Evaluated}
In this study, we evaluate the FRSs by AWS, Face++ and Microsoft for the following three tasks-
\begin{compactitem}
	\item Gender Detection: Each of the FRSs responds with either Male or Female gender for an input image, with AWS Rekognition also returning a confidence score for it's prediction.
	\item Age Prediction: AWS returns a window of size ranging from 10 to 18 years whereas both Face++ and Microsoft return whole numbers. Thus, we use the median value from AWS's prediction and the reported values from Microsoft and Face++. Further, we use a range of ground truth $\pm 4$ to check for the accuracy of prediction. Thus if the ground truth value is $20$ yrs, then according to our formula, the accuracy will be taken to be false if it lies outside the range $\lbrack 16, 24 \rbrack$ and true otherwise.
	\item Smile Detection: AWS responds with a Smile or No-smile label and a confidence score for its prediction. Face++ and Microsoft respond with a confidence value in $\lbrack 0,100 \rbrack$ and $\lbrack 0,1 \rbrack$ respectively. Thus we consider the threshold as $50\%$ and $0.5$ respectively to consider the prediction as true.
\end{compactitem}

\subsection{Datasets Evaluated}
In this study we have evaluated the following datasets-- \textsc{CelebSET} and \textsc{CFD} (and its extensions-- \textsc{CFD-MR} and \textsc{CFD-India}). The number of images in each dataset are as follows- \textsc{CelebSET}--1600, \textsc{CFD}--597, \textsc{CFD-MR}--88 and \textsc{CFD-India}--142. The filters applied on each dataset as well as the tasks evaluated are given in Table \ref{tab2:dataset-filter-tasks}.
\begin{table}
    \small
	\begin{center}
		\begin{tabular}{ c | c | c} 
			\textbf{Dataset} & \textbf{Filters} & \textbf{Tasks} \\
			\hline
			\textbf{\textsc{CelebSET}}\rule{0pt}{2ex} & Spread $|$ RGB & Gender $|$ Age $|$ Smile\\
			\hline
			\textbf{\textsc{CFD}}\rule{0pt}{2ex} & Newsprint $|$ Spread $|$ RGB & Gender $|$ Age \\
			\hline
		\end{tabular}
	\end{center}
	\caption{\textbf{Filters and Tasks for each dataset}}\label{tab2:dataset-filter-tasks}\todo{need to fix alignment}
\end{table}

\subsection{Experimental Setup}
We evaluate all datasets in batch mode through API calls to the FRS servers.
The parameter settings for each filter on \textsc{Gimp} are given as follows--
\begin{compactitem}
	\item \textbf{Spread}: Horizontal/Vertical Spread amount-- 50 units for \textsc{CFD} and 8 for \textsc{CelebSET}.
	\item \textbf{Newsprint}: Screen cell width-- 20 pixels, percentage of black pulled out-- $12\%$, screen angle for all colors-- 75$^{\circ}$
	\item \textbf{RGB}: Noise in RGB channels-- 0.8 for \textsc{CFD} and 0.5 for \textsc{CelebSET}.
\end{compactitem}

We now discuss the audit results for \textsc{CelebSET} and \textsc{CFD}.

\subsection{Observations for \textsc{CelebSET}}

\begin{table}
    \small
	\begin{center}
		\begin{tabular}{c | c | c | c} 
			\hline
			FRS\rule{0pt}{2ex} & Gender & Age & Smile \\ 
			\hline
			AWS\rule{0pt}{2ex} & $-0.25\%$& $-17.46\%$& $-5.54\%$ \\ 
			Microsoft\rule{0pt}{2ex} & $-0.63\%$ & $-21.22\%$ & $+12.94\%$ \\
			%			Face++\rule{0pt}{2ex} & $+9.1\%$ & X & X \\
			\hline
		\end{tabular}
	\end{center}
		\caption{\label{tab:celebset-old-new}\textbf{Change in accuracy for \textsc{CelebSET} relative to Saving Face\cite{raji2020saving}}}
\end{table}

\textsc{CelebSET} is a balanced dataset of 1600 images with an equal distribution of male and female individuals belonging to the following ethnic groups-- White Male(WM), White Female(WF), Black Male(BM) and Black Female(BF). 

The number of images identified by the FRSs are--
\begin{compactitem}
	\item \textbf{Original}-- AWS: 1600, Face++: 1600, Microsoft:1590
	\item \textbf{Spread Filter}-- AWS: 1549, Face++: 1534, Microsoft: 1552
	\item \textbf{RGB Filter}-- AWS: 20, Face++: 318, Microsoft: 683
\end{compactitem}

The above list shows that adding adversarial filters to low quality images successfully fools the FRS APIs. It is interesting to note that the RGB filter has an extremely high misclassification rate for all FRS with faces identified on less than $2\%$ images for AWS.

%This confirms our hypothesis that addition of simple filters elicits an adversarial response from the FRS APIs, with AWS identifying faces on less RGB-filter images .

\subsubsection{Change in Prediction Accuracy over time}
%\subsubsection{General Audit}
Table \ref{tab:celebset-old-new} shows the change in accuracy for the gender, age and smile prediction tasks as compared against the findings of Raji et al.\cite{raji2020saving}.

\textbf{Observation.}  From Table \ref{tab:celebset-old-new}, we can see that both AWS and Microsoft report a marginal drop in accuracy for gender detection by $0.25\%$ and $0.63\%$ respectively. The drop in accuracy for age prediction is even worse at $\approx 17.5\%$ for AWS and $\approx 21\%$ for Microsoft. Interestingly, while AWS has also worsened for Smile detection, Microsoft has improved by a significant $\approx 13\%$.

\textbf{Key Takeaways.}
\begin{compactitem}
	\item The FRSs have degraded in their performance over time.
	\item Overcompensation by improvement in accuracy for one feature significantly impacts the accuracy for another task as seen for Microsoft.
\end{compactitem}

% \subsubsection{Change in Accuracy from previous audits}\todo{fix when KD shares new numbers for Table \ref{tab:celebset-old-new} }
% %\subsubsection{General Audit}
% Table \ref{tab:celebset-old-new} shows the change in accuracy for the gender, age and smile prediction tasks as compared against the findings of Raji et al.\cite{raji2020saving}. We can see that both AWS and Microsoft have marginally degraded in the accuracy for the gender detection task, and significantly for the age prediction task since the previous audit. It is interesting to note that while AWS now performs worse on the smile prediction task, Microsoft has improved by a significant $\approx 13\%$. This leads to the following observations--
% \begin{itemize}
% 	\item Improvement of accuracy in one task can affect the accuracy for another task and based on the use case, this might lead to unfair outcomes.
% 	\item The accuracy of commercial FRS keeps changing with time. In the interest of transparency and protecting users from facing biased outcomes, these vendors should submit these commercial systems to regular benchmarked third-party audits with results being publicly available so that users are aware of the current level of bias in these software and can make an informed decision before using them. We also propose that each of these FRS vendors should release model cards \cite{mitchell2019model} to increase transparency and understanding of their systems among the community.
% \end{itemize}

We next discuss the prediction accuracy for the three FRS APIs over the tasks of Gender, Age and Smile predicition for the original as well as adversarial inputs. We also study the bias between the intersectional groups for the same.

%\subsubsection{Prediction Accuracy for Adversarial Inputs}
\subsubsection{Overall Prediction Accuracy}

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.66\columnwidth}
		%\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/AWS_G_A_S_CLBST-new.pdf}
		% 		\vspace*{-2mm}
		\caption{Accuracy on AWS}
		\label{Fig: AWS-celebset-accuracy}
	\end{subfigure}%
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/FPP_G_A_S_CLBST-new.pdf}
		% 		\vspace*{-2mm}
		\caption{Accuracy on Face++}
		\label{Fig: FPP-celebset-accuracy}
	\end{subfigure}
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/MSFT_G_A_S_CLBST-new.pdf}
		% 		\vspace*{-2mm}
		\caption{Accuracy on Microsoft}
		\label{Fig: MSFT-celebset-accuracy}
	\end{subfigure}
	
	%\vspace*{-4mm}
	\caption{{\bf Prediction Accuracy on \textsc{CelebSET} for Original, RGB-filter and Spread-Filter inputs. Under adversarial settings, all the FRSs suffer from drop in accuracy(AWS has $\bf < 2\%$ accuracy), with Microsoft being marginally more robust than AWS and Face++.}}
	\label{fig:celebset-accuracy}
	%\vspace{-4 mm}
\end{figure*}

\begin{table*}[!ht]
    \small
	\begin{center}
		\begin{tabular}{c | c | c | c} 
			\hline
			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} & \textbf{Smile}\\
			\hline
			AWS/Original\rule{0pt}{2ex} & \textbf{(WF - WM)} $1\%$ & \textbf{(WF - BF)} $19.25\%$ & \textbf{(BF - WM)} $6.5\%$ \\ 
			AWS/RGB\rule{0pt}{2ex} & \textbf{(WM - BM/BF)} $1.75\%$ & \textbf{(WM - BM)} $1.25\%$ & \textbf{(BF - BM)} $1.25\%$ \\
			AWS/Spread\rule{0pt}{2ex} & \textbf{(WF - WM)} $\textbf{5.5\%}$ & \textbf{(WF - BF)} $\textbf{19.5\%}$ & \textbf{(BF - WM)} $\textbf{12.5\%}$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{4.5\%(Spread)} & \cellcolor{red!20} \textbf{0.5\%(Spread)} & \cellcolor{red!20} \textbf{6\%(Spread)}\\
			\hline
			Face++/Original\rule{0pt}{2ex} & \textbf{(WM - BF)} $2.5\%$ & \textbf{(WF - WM)} $\textbf{13.5\%}$ & \textbf{(BF - BM)} $7\%$ \\ 
			Face++/RGB\rule{0pt}{2ex} & \textbf{(WF - BM)} $\textbf{22.75\%}$ & \textbf{(BF - BM)} $4.25\%$ & \textbf{(WF - BM)} $\textbf{20.75\%}$ \\
			Face++/Spread\rule{0pt}{2ex} & \textbf{(WF - BM)} $17.5\%$ & \textbf{(BM - WM)} $2.5\%$ & \textbf{(WF - BM)} $12.5\%$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{20.25\%(RGB)} & \cellcolor{red!20} $\phi$ & \cellcolor{red!20} \textbf{13.75\%(RGB)}\\
			\hline
			Microsoft/Original\rule{0pt}{2ex} & \textbf{(WM/WF - BM/BF)} $1\%$ & \textbf{(BM - BF)} $16\%$ & \textbf{(WF - BM)} $4.5\%$ \\ 
			Microsoft/RGB\rule{0pt}{2ex} & \textbf{(WF - BM/BF)} $\textbf{36.25\%}$ & \textbf{(WF - BM)} $15.75\%$ & \textbf{(WF - BM)} $\textbf{33.75\%}$ \\
			Microsoft/Spread\rule{0pt}{2ex} & \textbf{(WF - BM/BF)} $6.5\%$ & \textbf{(WM - BF)} $\textbf{30\%}$ & \textbf{(WF - BM)} $9.5\%$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{35.25\%(RGB)} & \cellcolor{red!20} \textbf{14\%(Spread)} & \cellcolor{red!20} \textbf{29.25\%(RGB)}\\
			\hline
		\end{tabular}
	\caption{\label{tab:celebset-intersection}\textbf{Difference in highest accuracy and lowest accuracy amongst the intersectional groups for \textsc{CelebSET}. Most results show significant disparity in prediction accuracy for people of `Black' ethnicity (BF/BM) as compared to that of `White'  ethnicity. Microsft reports the largest disparity for all tasks, irrespective of the input.}}
	\end{center}
\end{table*}

Figure \ref{fig:celebset-accuracy} presents the prediction accuracy for the three tasks of Gender, Age and Smile Detection. Each of the plots- Fig. \ref{Fig: AWS-celebset-accuracy}, \ref{Fig: FPP-celebset-accuracy} and \ref{Fig: MSFT-celebset-accuracy} correspond to an FRS API. 

\textbf{Observations.}
We can see that all FRS APIs report high gender identification accuracies ($\geq 99\%$) for the original dataset. With the adversarial filters, this accuracy is significantly affected, with AWS reporting an accuracy of only $1.5\%$ (Fig. \ref{Fig: AWS-celebset-accuracy}). The drop in accuracy for Spread filter is not as significant with the lowest reported accuracy being $92\%$ for Face++ (Fig. \ref{Fig: FPP-celebset-accuracy}).

For the task of age prediction, all APIs perform badly even for the original input with only Microsoft having an accuracy of $ > 50\%$ (Fig. \ref{Fig: MSFT-celebset-accuracy}). The adversarial filters reduce this even further with RGB filter causing a drop of $ > 50\%$. Here again, Face++ has the lowest accuracy for Spread filter--  $\approx 28\%$ (Fig. \ref{Fig: FPP-celebset-accuracy}).

Finally, all APIs are able to identify smiles with an accuracy of ($\geq 88\%$) for the original dataset, but exhibit a similar behaviour for the accuracy on RGB and Spread filters, with Microsoft being the best overall and AWS being the worst. 

\textbf{Key Takeaways.}
The key takeaways from Figure \ref{fig:celebset-accuracy} are as follows--
\begin{compactitem}
	\item All FRS APIs perform well on the original input for Gender and Smile but badly for Age detection.
	\item All FRS APIs perform badly for RGB filter with AWS being the worst but comparatively better for Spread filter with Face++ being the worst.
	\item Microsoft is best performing FRS overall across all tasks and inputs.
\end{compactitem}

%\textbf{Gender Detection.} All APIs perform extremely well for the gender identification task over the original dataset with an accuracy of $\geq 99\%$. When the RGB-filtered images are provided as input, the performance is impacted significantly- dropping to $1\%$ for AWS. The Spread filter images too are impacted but the drop in accuracy is not as significant, with Face++ being the worst at $92\%$. Thus, RGB-filters are clearly able to fool the APIs into either not detecting the faces, or detecting the genders incorrectly for most inputs.
%
%\textbf{Age Prediction.} For this task, all APIs perform badly, with only Microsoft having an accuracy of $ > 50\%$. The adversarial inputs have a similar impact on the accuracy of this task with the APIs performing worst on RGB-filter images. Here again Microsoft performs best with an accuracy of $16\%$ for RGB-filter images and $\approx 41\%$ for Spread-filter images.
%
%\textbf{Smile Detection.} All APIs perform well on this task over both the original images and the Spread-filter images, with Microsoft giving the best accuracy of $93\%$ and $90\%$ respectively. Once again it can be observed that the APIs perform the worst on the RGB-filter images with AWS being the worst at $\approx 0.8\%$.
%
%From these results, we can conclude that both the filters affect the accuracies for all APIs with RGB having a greater impact than Spread. Overall, Microsoft has the best accuracy on the adversarial images and AWS has the worst.

%\subsubsection{Bias over Intersectional Groups}
\subsubsection{Disparity in Accuracy for intersectional Groups}
We now evaluate the disparity in accuracy by taking the difference of the highest accuracy and the lowest accuracy among the different intersectional groups- WM, WF, BM, BF. The results are in Table \ref{tab:celebset-intersection}.

\textbf{Observations.} For the task of gender detection, we can see that the disparity increases for the two adversarial filters for all FRS APIs with a maximum of $36.25\%$ for Microsoft/RGB. This disparity is mostly against people of `Black' ethnicity as compared to people of `White' ethnicity. Infact, it is highest for Microsoft despite its accuracy being highest amongst the three systems (Fig. \ref{fig:celebset-accuracy}).

The disparity amongst the different intersectional groups for age prediction is slightly lower with a maximum value of $30\%$ for Microsoft/Spread. Interestingly the disparity reduces for all FRS APIs for the RGB filter with Face++ infact reporting a decrease in the measure. Here again, the ethnicity that is most biased against is `Black'.

Finally, for smile detection we can see that both Face++ and Microsoft report the highest disparity for RGB filter and AWS for Spread. The largest disparity is $33.75\%$, reported by Microsoft for RGB filter images. It also has the maximum absolute increase in disparity.


\textbf{Key Takeaways.}
The key takeaways from the observations for intersectional disparity on \textsc{CelebSET} are--
\begin{itemize}
	\item All FRSs exhibit an increase in disparity of accuracy for both Gender and Smile detection, with only Age Prediction reporting a decrease in disparity for some instances.
	\item There is a noticeable and significant disparity in accuracy against individuals of `Black' ethnicity.
	\item Even though Microsoft reports the highest accuracies amongst the three FRSs, the disparities between the two ethnicities are also the highest. Thus the high accuracy comes at the cost of increased bias.
\end{itemize}
%For AWS, it can be clearly seen that the difference in accuracy between the different intersectional groups increases for the Spread Filter as compared against the original images for all the tasks under consideration. As the number of images identified for RGB-filter are so low, the results for this should not be considered significant.
%
%Similarly, we can see that for Face++/RGB the bias for gender detection increases from $2.5\%$ to $22.75\%$ and for smile detection increases from $7\%$ to $20.75\%$. Surprisingly the bias in age prediction reduces from $13.5\%$ to as low as $2.5\%$ for the Spread-filter.
%
%For Microsoft, we have similar observations as Face++ with the bias for RGB increasing by $30\times$ for gender detection task and by $8\times$ for smile detection task. The bias for age also doubles when the Spread-filter images are considered. Microsoft shows a clear trend of bias against dark-skinned individuals irrespective of the task being considered.
%
%This table shows that adversarial inputs affect not just the accuracy but also the bias amongst different intersectional groups which show a steep increase. Another important observation is that across the three FRS APIs and the tasks, the difference in accuracy is widest between lighter skinned females and darker skinned females.

We observe similar results for biases between genders and ethnicities for the three tasks. The results have been ommitted for brevity.

\subsection{Observations for \textsc{CFD}}
We also perform a similar audit as \textsc{CelebSET}, on \textsc{CFD}. This dataset has higher quality images with standardized lighting and face angles and has individuals belonging to four different ethnicities-- `White', `Black', `Latino', `Asian'. AWS and Microsoft APIs are able to identify faces in all 597 images but Face++ identifies only 423 images with faces for the Newsprint filter. 


%Along with \textsc{CelebSET}, we performed an audit on the same set of FRS APIs using another database of images- \textsc{CFD}. The reasons for choosing this dataset were primarily--
%\begin{itemize}
%	\item High quality professionally shot photographs with consistent lighting and angle.
%	\item More ethnicities were covered- Latino and Asian.
%\end{itemize}
%
%This introduced a different kind of challenge into our study as we were able to test for adversarial inputs over high resolution images. Here, 
%We now discuss the results for accuracy and intersectional bias for the three FRS APIs on this dataset. For the sake of brevity, we have ommitted a detailed discussion of intersectional bias on CFD-MR and CFD-India in the current submission.

\subsubsection{Overall Prediction Accuracy}
\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.66\columnwidth}
		%\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/AWS_G_A_S_CFD_USA-new.pdf}
		% 		\vspace*{-4mm}
		\caption{Accuracy on AWS}
		\label{Fig: AWS-cfd-accuracy}
	\end{subfigure}%
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/FPP_G_A_S_CFD_USA-new.pdf}
		%\vspace*{-3.5mm}
		\caption{Accuracy on Face++}
		\label{Fig: FPP-cfd-accuracy}
	\end{subfigure}
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/MSFT_G_A_S_CFD_USA-new.pdf}
		%\vspace*{-3.5mm}
		\caption{Accuracy on Microsoft}
		\label{Fig: MSFT-cfd-accuracy}
	\end{subfigure}
	
	%\vspace*{-4mm}
	\caption{{\bf Prediction Accuracy on \textsc{CFD} for Original, RGB-filter, Newsprint-filter and Spread-Filter inputs. Under RGB and Newsprint adversarial settings, all of the FRTs suffer from drop in accuracy (Face++ accuracy drops by $\bf > 50\%$), with Microsoft being marginally more robust than AWS and Face++.}}
	\label{fig:cfd-accuracy}
	%\vspace{-4 mm}
\end{figure*}

The prediction accuracy results for the tasks of Gender and Age detection are presented in
Figure \ref{fig:cfd-accuracy}. The results are divided per FRS API in Figs. \ref{Fig: AWS-cfd-accuracy}, \ref{Fig: FPP-cfd-accuracy} and \ref{Fig: MSFT-cfd-accuracy}.

\textbf{Observations.}
All FRS APIs report a high accuracy for the task of gender detection, with Microsoft $\geq 99\%$ (Fig. \ref{Fig: MSFT-cfd-accuracy}). Even with the adversarial Spread filter, we do not observe any drop in accuracy. With other adversarial filters like RGB and Newsprint, we observe a noticeable drop in accuracy, with AWS and Face++ reporting a drop of $\geq 40\%$ (Figs. \ref{Fig: AWS-cfd-accuracy}, \ref{Fig: FPP-cfd-accuracy}) for Newsprint. Microsoft is the best performing API here with a minimum accuracy of $\approx 96\%$ across all inputs.

%We can see that all FRS APIs report high gender identification accuracies ($\geq 99\%$) for the original dataset. With the adversarial filters, this accuracy is significantly affected, with AWS reporting an accuracy of only $1.5\%$ (Fig. \ref{Fig: AWS-celebset-accuracy}). The drop in accuracy for Spread filter is not as significant with the lowest reported accuracy being $92\%$ for Face++ (Fig. \ref{Fig: FPP-celebset-accuracy}).

Age prediction accuracy is low for all FRS APIs irrespective of the input. Here, Face++ is the worst performing system with the accuracies lying between $\approx 14\%$ for Face++/RGB and $\approx 47\%$ for Face++/Spread (Fig. \ref{Fig: FPP-cfd-accuracy}). Microsoft, on the other hand, returns the best results with its reported accuracies in the range $\approx 62\%$ to $\approx 77\%$ (Fig. \ref{Fig: MSFT-cfd-accuracy}).

%For the task of age prediction, all APIs perform badly even for the original input with only Microsoft having an accuracy of $ > 50\%$ (Fig. \ref{Fig: MSFT-celebset-accuracy}). The adversarial filters reduce this even further with RGB filter causing a drop of $ > 50\%$. Here again, Face++ has the lowest accuracy for Spread filter--  $\approx 28\%$ (Fig. \ref{Fig: FPP-celebset-accuracy}).

%Finally, all APIs are able to identify smiles with an accuracy of ($\geq 88\%$) for the original dataset, but exhibit a similar behaviour for the accuracy on RGB and Spread filters, with Microsoft being the best overall and AWS being the worst. 

\textbf{Key Takeaways.}
The key takeaways from the above results are as follows--
\begin{itemize}
	\item All APIs perform well for the task of gender detection for all inputs except Newsprint, while the performance for age prediction is bad for all inputs on AWS and Face++.
	\item Face++ is the worst performing FRS for both Gender and Age prediction.
	\item Microsoft is best performing FRS overall across all tasks and inputs.
\end{itemize}
%We present the results for accuracy of prediction for the tasks of gender and age detection in Figure \ref{fig:cfd-accuracy}. The three plots correspond to each FRS API with each cluster of bars corresponding to a task. 

%\textbf{Gender Detection.} All APIs perform extremely well for the gender identification task over the original dataset with an accuracies ranging from $\approx 93\%$ for Face++ to $ > 99\%$ for Microsoft. For the RGB-filtered images, the lowest accuracy is reported by Face++ at $\approx 89\%$ with Microsoft performing the best at $\approx 98.5\%$ accuracy. Thus, contrary to \textsc{CelebSET}, this dataset does not get impacted by RGB-filter despite having a higher value of noise (0.8 compared to 0.5). Experimenting with the Newsprint filter, exposes the shortcomings of the AWS and Face++ API, as both experience a sharp drop in accuracy by almost $50\%$, although Microsoft seems to deal with challenge well enough reporting only a $2.5\%$ drop in accuracy.

%\textbf{Age Prediction.} For this task, Microsoft perform well on the initial dataset but Face++ reports an accuracy less than $50\%$. For the adversarial inputs, Microsoft is again the best performing API with a drop in accuracy of only $6.8\%$ for RGB and $15\%$ for Newsprint. Here again, Face++ is the worst performing API with its accuracy going as low as $\approx 14\%$ for RGB-filter images.
Thus, we see a consistent trend of API performances being impacted because of these simple filters.

\begin{table*}[!ht]
    \small
	\begin{center}
%		\caption{\label{tab:cfd-ethnic}Difference in Accuracy between different ethnic groups for \textsc{CFD}}
		\begin{tabular}{c | c | c } 
			\hline
			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} \\
			\hline
			AWS/Original\rule{0pt}{2ex} & \textbf{(W - B)} $3.48\%$& \textbf{(W - B)} $\textbf{23.64\%}$ \\ 
			AWS/RGB\rule{0pt}{2ex} & \textbf{(A - B)} $8.93\%$ & \textbf{(W - B)} $15.83\%$ \\
			AWS/Newsprint\rule{0pt}{2ex} & \textbf{(A - B)} $\textbf{14.45\%}$ & \textbf{(A - B)} $22.66\%$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{10.97\%(Newsprint)} & \cellcolor{red!20} $\phi$\\			
			\hline
			Face++/Original\rule{0pt}{2ex} & \textbf{(A - B)} $8.93\%$& \textbf{(L - W)} $7.67\%$ \\ 
			Face++/RGB\rule{0pt}{2ex} & \textbf{(L - W)} $8.48\%$ & \textbf{(B - A)} $7.68\%$ \\
			Face++/Newsprint\rule{0pt}{2ex} & \textbf{(L - B)} $\textbf{36.89\%}$ & \textbf{(L - B)} $\textbf{38.83\%}$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{27.96\%(Newsprint)} & \cellcolor{red!20} \textbf{31.16\%(Newsprint)}\\
			\hline
			Microsoft/Original\rule{0pt}{2ex} &\textbf{(W/L/A - B)} $0.51\%$& \textbf{(A - B)} $\textbf{15.37\%}$\\ 
			Microsoft/RGB\rule{0pt}{2ex} & \textbf{(L/A - B)} $2.54\%$ & \textbf{(L - B)} $15.16\%$ \\
			Microsoft/Newsprint\rule{0pt}{2ex} & \textbf{(A - B)} $\textbf{4.26\%}$ & \textbf{(A - B)} $13.38\%$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{3.75\%(Newsprint)} & \cellcolor{red!20} $\phi$\\
			\hline
		\end{tabular}
	\end{center}
	\caption{\label{tab:cfd-ethnic}\textbf{Difference in highest accuracy and lowest accuracy amongst the ethnic groups for \textsc{CFD}. Most results show significant disparity in prediction accuracy for people of `Black' ethnicity as compared to that of other ethnicities. Face++ reports the largest disparity for all tasks on the Newsprint adversarial input.}}
\end{table*}

%\subsubsection{Bias over Ethnic Groups}
\subsubsection{Disparity in Accuracy for Ethnic Groups}
We now evaluate the disparity in accuracy by taking the difference of the highest accuracy and the lowest accuracy among the different ethnic groups- `White', `Black', `Latino', `Asian'. The results are in Table \ref{tab:cfd-ethnic}.

\textbf{Observations.} We see that for the task of gender detection, AWS and Face++ report extremely high disparities with the Newsprint filter-- $\approx 14.5\%$ and $\approx 36.9\%$ respectively. This is in contrast to Microsoft which has a disparity of only $\approx 4\%$. The interesting observation here is that all the FRSs report this disparity against the `Black' ethnic group. Thus Face++ has both the lowest accuracy as well as the highest disparity.

For the task of age prediction, both AWS and Microsoft report a drop in disparity with only Face++ reporting an increase of over $30\%$. Here again, the disparities mostly exist against the `Black' ethnic group.

\textbf{Key Takeaways.}
The key takeaways from the observations for intersectional disparity on \textsc{CelebSET} are--
\begin{itemize}
	\item All FRSs exhibit an increase in disparity of accuracy for Gender detection, with only Face++ Prediction reporting an increase for age prediction.
	\item There is a noticeable and significant disparity in accuracy against individuals of `Black' ethnicity.
	\item Face++ reports the least accuracy as well as the highest bias. AWS and Microsoft exhibit all disparities against the `Black' ethnic group.
\end{itemize}


%We now evaluate the change in bias due to these adversarial inputs by evaluating the difference in accuracies between the following ethnic groups- W, B, L and A in Table \ref{tab:cfd-ethnic}. The percentage values in bold are the highest within a particular group. 

%For all APIs, it can be seen that for the task of Gender Detection, the bias increases with the usage of adversarial inputs with Face++/RGB being the only exception. Another concerning observation is that individuals belonging to the Black community suffer the most discrimination even for adversarial inputs and this bias only increases, going as high as $\approx 37\%$ for Face++/Newsprint. Although Microsoft reports the least discrimination it is still directed towards one particular ethnic group irrespective of the type of filter applied.
%
%Interestingly, for the age prediction task we can see that only Face++ reports an increase in bias with both AWS and Microsoft infact reporting a reduction in bias. Here too we notice that the Black ethnicity individuals are most discriminated against and the increase in bias in Face++ is a significant $\approx 39\%$ against the same.
%
%This table clearly shows that even though there has been an improvement in accuracy for age detection by the various APIs, there is still a very heavy bias against particular ethnicities and this only gets enhanced in adversarial scenarios.

We observe similar results for biases between genders, the results for which have been omitted for brevity.

\begin{table*}[!ht]
    \small
	\begin{center}
%		\caption{\label{tab:cfd-intersection}Difference in Accuracy between different intersectional groups for \textsc{CFD}}
		\begin{tabular}{c | c | c } 
			\hline
			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} \\
			\hline
			AWS/Original\rule{0pt}{2ex} & \textbf{(WF/LM/AM - BF)} $7.69\%$& \textbf{(WM - BM)} $33.33\%$ \\ 
			AWS/RGB\rule{0pt}{2ex} & \textbf{(BM - BF)} $20.07\%$ & \textbf{(WF - AF)} $24.16\%$ \\
			AWS/Newsprint\rule{0pt}{2ex} & \textbf{(WF - BM)} $\textbf{71.82\%}$ & \textbf{(LF - LM)} $\textbf{42.72\%}$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{64.13\%(Newsprint)} & \cellcolor{red!20} \textbf{9.39\%(Newsprint)}\\		
			\hline
			Face++/Original\rule{0pt}{2ex} & \textbf{(WM/LM/AM - BF)} $21.25\%$ & \textbf{(LM - WF)} $28.80\%$ \\ 
			Face++/RGB\rule{0pt}{2ex} & \textbf{(WF/LF/AF - WM)} $25.81\%$ & \textbf{(BM - AF)} $21.91\%$ \\
			Face++/Newsprint\rule{0pt}{2ex} & \textbf{(LM - BF)} $\textbf{93.27\%}$ & \textbf{(LF - BM)} $\textbf{44.26\%}$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{72.02\%(Newsprint)} & \cellcolor{red!20} \textbf{15.46\%(Newsprint)}\\
			\hline
			Microsoft/Original\rule{0pt}{2ex} & \textbf{(WM/WF/BM/LM/LF/AM/AF - BF)} $0.96\%$& \textbf{(AF - BF)} $\textbf{25.22\%}$ \\ 
			Microsoft/RGB\rule{0pt}{2ex} & \textbf{(BM/LM/LF/AM/AF - BF)} $4.81\%$ & \textbf{(LF - BF)} $21.57\%$ \\
			Microsoft/Newsprint\rule{0pt}{2ex} & \textbf{(BM/LF - BF)} $\textbf{11.54\%}$ & \textbf{(WM - BF)} $21.08\%$ \\
			\cellcolor{red!20}Max. absolute increase in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{10.58\%(Newsprint)} & \cellcolor{red!20} $\phi$\\
			\hline
		\end{tabular}
	\end{center}
	\caption{\label{tab:cfd-intersection}\textbf{Difference in highest accuracy and lowest accuracy amongst the intersectional groups for \textsc{CFD}. Most results show significant disparity in prediction accuracy for people of `Black' ethnicity (BF/BM) as compared to that of other ethnicities. Face++ reports the largest disparity for all tasks on the Newsprint adversarial input.}}
\end{table*}

\if 0 
\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.66\columnwidth}
		%\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/AWS_G_A_S_CFD_MR-new.pdf}
		% 		\vspace*{-4mm}
		\caption{Accuracy on AWS}
		\label{Fig: AWS-cfd-mr-accuracy}
	\end{subfigure}%
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/FPP_G_A_S_CFD_MR-new.pdf}
		%\vspace*{-3.5mm}
		\caption{Accuracy on Face++}
		\label{Fig: FPP-cfd-mr-accuracy}
	\end{subfigure}
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/MSFT_G_A_S_CFD_MR-new.pdf}
		%\vspace*{-3.5mm}
		\caption{Accuracy on Microsoft}
		\label{Fig: MSFT-cfd-mr-accuracy}
	\end{subfigure}
	
	%\vspace*{-4mm}
	\caption{{\bf Performance on \textsc{CFD-MR} for Original, RGB-Filter and Newsprint-filter inputs }}
	\label{fig:cfd-mr-accuracy}
	%\vspace{-4 mm}
\end{figure*}
\fi 
%\subsubsection{Bias over Intersectional Groups}
\subsubsection{Disparity in Accuracy for Intersectional Groups}
Here, we discuss the disparity in accuracy amongst the eight different intersectional groups formed by taking male and female members from each of the ethnic group- `White', `Black', `Latino', `Asian'. The results are presented in Table \ref{tab:cfd-intersection}.

\textbf{Observations.} The results in Table \ref{tab:cfd-intersection} go one level deeper and show that for the task of gender identifcation, people belonging to `Black' ethnicity, specially females, experience the highest disparity, irrespective of the type of input. AWS reports a disparity of $\approx 72\%$ and Face++ reports a disparity of $\approx 93\%$ with Microsoft a distant third at $11.5\%$, on the Newsprint filter. This shows the adversarial nature of the Newsprint filter affecting all FRSs with Face++ affected the most.

For age prediction, while all FRSs report a drop in disparity for the RGB filter, AWS and Face++ report an increase for Newsprint, with Face++ reporting the  highest disparity at $44\%$. Here, Microsoft always exhibits disparity against `Black' females whereas AWS and Face++ show slightly different behaviour, with other minority groups too experiencing disparate accuracy.

\textbf{Key Takeaways.}
The key takeaways from the observations for intersectional disparity on \textsc{CelebSET} are--
\begin{itemize}
	\item All FRSs exhibit an increase in disparity of accuracy for Gender detection, mostly directed towards individuals of `Black' ethnicity.
	\item Face++ reports the highes disparity for all experiments with a value of $93.27\%$ between `Latino' males and `Black' females.
	\item Microsoft is the best performing FRS, yet it is the most disparate against `Black' females, with all its lowest accuracies being reported for this group.
\end{itemize}


%Finally, we evaluate the change in bias for the different intersectional groups in this dataset as shown in Table \ref{tab:cfd-intersection}. 

%For all APIs, it is clear that the bias in gender detection task between intersectional groups increases in the order-- Original < RGB-filter < Newsprint-filter. Another common trend for all APIs is that the bias is against people belonging to the Black ethnicity with more bias against the females as compared to the males. For AWS, this increases from $~7.6\%$ to $71.8\%$ whereas it goes as high as $93.3\%$ for Face++/Newsprint. In comparison, Microsoft performs significantly better with a maximum bias of $11.5\%$. 
%
%For the task of age prediction it is observed that the bias decreases between the original images and the images with RGB filter for all APIs. For the Newsprint-filter, AWS and Face++ report an increase in bias whereas Microsoft reports the least bias. Here again we can see that the bias is mostly against people of Black ethnicity with only Face++ being an exception.
%
%These results show that photographs of better quality and resolution may infact report higher biases against dark skinned individuals and therefore should be considered even more concerning and confirm the fact that Facial Analysis software is far from perfect and with the commonplace use of simple filters may infact be propagating more biased responses which can have significant ramifications in the long term.


\subsection{Observations for \textsc{CFD-MR} and \textsc{CFD-India}}
Along with \textsc{CFD}, we have also evaluated two other datasets- \textsc{CFD-MR} and \textsc{CFD-India}. These are newly released datasets and allow us to study disparities in accuracy for ethnicities that are not generally studied in the context of FRS audits. 
%\subsubsection{Prediction Accuracy for Adversarial Inputs}

\subsubsection{Disparity in Accuracy between Males and Females}
\if 0 
\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.66\columnwidth}
		%\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/AWS_G_A_S_CFD_IND-new.pdf}
		% 		\vspace*{-4mm}
		\caption{Accuracy on AWS}
		\label{Fig: AWS-cfd-ind-accuracy}
	\end{subfigure}%
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/FPP_G_A_S_CFD_IND-new.pdf}
		%\vspace*{-3.5mm}
		\caption{Accuracy on Face++}
		\label{Fig: FPP-cfd-ind-accuracy}
	\end{subfigure}
	~\begin{subfigure}{0.66\columnwidth}
		\centering
		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/MSFT_G_A_S_CFD_IND-new.pdf}
		%\vspace*{-3.5mm}
		\caption{Accuracy on Microsoft}
		\label{Fig: MSFT-cfd-ind-accuracy}
	\end{subfigure}
	
	%\vspace*{-4mm}
	\caption{{\bf Performance on \textsc{CFD-India} for Original, RGB-Filter and Newsprint-filter inputs }}
	\label{fig:cfd-ind-accuracy}
	%\vspace{-4 mm}
\end{figure*}
\fi 
%We present the results for accuracy of prediction for the tasks of gender and age detection for \textsc{CFD-MR} in Figure \ref{fig:cfd-mr-accuracy} and for \textsc{CFD-India} in Figure \ref{fig:cfd-ind-accuracy}. 

%\textbf{Gender Detection.} For both the datasets, we see that all APIs have an accuracy of $> 90\%$ with Microsoft reporting an accuracy of $100\%$ for both the datasets. Here, Face++ is the weakest FRS with an accuracy of $\approx 90\%$ for \textsc{CFD-MR}(Figure \ref{Fig: FPP-cfd-mr-accuracy}) and $\approx 92\%$ for \textsc{CFD-India}(Figure \ref{Fig: FPP-cfd-ind-accuracy}). 
%For RGB-filtered images, the accuracy drop is minimal with Face++ infact reporting an increase in accuracy for \textsc{CFD-India} as can be seen in Figure \ref{Fig: FPP-cfd-ind-accuracy}. Thus similar to CFD-USA, these datasets also don't get impacted by RGB-filter.
%For Newsprint-filter we notice a significant drop in accuracy for both AWS and Face++ APIs, but almost no drop in accuracy for Microsoft. Face++ reports a drop in accuracy to $\approx 20.4\%$ in Figure \ref{Fig: FPP-cfd-mr-accuracy}. A similiar drop in accuracy is observed for both AWS and Face++ in \textsc{CFD-India} as well from Figures \ref{Fig: AWS-cfd-ind-accuracy} and \ref{Fig: FPP-cfd-ind-accuracy}.

%\textbf{Age Prediction.} Similar to \textsc{CFD}, Microsoft is the best performing API here and Face++ the worst, for both the datasets. The behaviour of the APIs for the different filters does not follow any pattern here, with Face++ reporting a lesser accuracy for RGB-filter than for Newsprint-filter (Figures \ref{Fig: FPP-cfd-mr-accuracy}, \ref{Fig: FPP-cfd-ind-accuracy}). AWS and Microsoft report alternating behaviour(ref. Figures \ref{Fig: AWS-cfd-mr-accuracy} and \ref{Fig: MSFT-cfd-mr-accuracy}, and Figures \ref{Fig: AWS-cfd-ind-accuracy} and \ref{Fig: MSFT-cfd-ind-accuracy}. The lowest accuracy is reported by Face++ for RGB-filter on \textsc{CFD-India} at $13.4\%$.

%Thus, we can see here that even with varied ethnicities, there is an impact on the accuracy of prediction for adversarial inputs.
%Here as well, Microsoft has the best accuracy on the adversarial images and Face++ has the worst.

\begin{table*}[!ht]
	\centering
	\begin{subtable}{.4\linewidth}
		\small
		\centering
		\begin{tabular}{c | c | c } 
			\hline
			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} \\
			\hline
			AWS/Original\rule{0pt}{2ex} & $3.23\%$ & $-10.04\%$ \\ 
			AWS/RGB\rule{0pt}{2ex} &  $-2.24\%$ & $7.69\%$ \\
			AWS/Newsprint\rule{0pt}{2ex} &  $\textbf{-63.65\%}$ &  $\textbf{-11.91\%}$ \\
			\cellcolor{red!20}Max. abs. inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{66.88\%(Newsprint)} & \cellcolor{red!20} \textbf{17.73\%(RGB)}\\
			\hline
			Face++/Original\rule{0pt}{2ex} & $12.90\%$ & $4.84\%$ \\ 
			Face++/RGB\rule{0pt}{2ex} & $-19.85\%$ & $8.93\%$ \\
			Face++/Newsprint\rule{0pt}{2ex} &  $\textbf{69.23\%}$ & $\textbf{29.03\%}$ \\
			\cellcolor{red!20}Max. abs. inc in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{56.33\%(Newsprint)} & \cellcolor{red!20} \textbf{24.19\%(Newsprint)}\\
			\hline
			Microsoft/Original\rule{0pt}{2ex} & $0\%$&  $\textbf{18.12\%}$ \\ 
			Microsoft/RGB\rule{0pt}{2ex} &  $0\%$ &  $17.49\%$ \\
			Microsoft/Newsprint\rule{0pt}{2ex} &  $0\%$ &  $-7.2\%$ \\
			\cellcolor{red!20}Max. abs. inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{$\phi$} & \cellcolor{red!20} \textbf{25.36\%(Newsprint)}\\
			\hline
		\end{tabular}
	\caption{\textsc{CFD-MR}}\label{tab:cfd-mr-gender}
	\end{subtable}%
\\
	\begin{subtable}{.4\linewidth}
		\small
		\centering
		\begin{tabular}{c | c | c } 
			\hline
			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} \\
			\hline
			AWS/Original\rule{0pt}{2ex} & $3.85\%$ & $15.77\%$ \\ 
			AWS/RGB\rule{0pt}{2ex} &  $7.69\%$ & $\textbf{23.08\%}$ \\
			AWS/Newsprint\rule{0pt}{2ex} &  $\textbf{-58.16\%}$ &  $-16.75\%$ \\
			\cellcolor{red!20}Max. abs inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{62.01\%(Newsprint)} & \cellcolor{red!20} \textbf{32.52\%(Newsprint)}\\			
			\hline
			Face++/Original\rule{0pt}{2ex} & $19.23\%$ & $4.36\%$ \\ 
			Face++/RGB\rule{0pt}{2ex} & $-0.30\%$ & $\textbf{-9.23\%}$ \\
			Face++/Newsprint\rule{0pt}{2ex} &  $\textbf{62.90\%}$ & $-1.07\%$ \\
			\cellcolor{red!20}Max. abs inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{43.67\%(Newsprint)} & \cellcolor{red!20} \textbf{13.59\%(RGB)}\\
			\hline
			Microsoft/Original\rule{0pt}{2ex} & $0\%$&  $-0.64\%$ \\ 
			Microsoft/RGB\rule{0pt}{2ex} &  $0\%$ &  $5.56\%$ \\
			Microsoft/Newsprint\rule{0pt}{2ex} &  $\textbf{1.92\%}$ & $\textbf{17.48\%}$ \\
			\cellcolor{red!20}Max. abs inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{1.92\%(Newsprint)} & \cellcolor{red!20} \textbf{18.12\%(Newsprint)}\\
			\hline
		\end{tabular}
		\caption{\textsc{CFD-India}}\label{tab:cfd-india-gender}
	\end{subtable}
%\caption{\label{tab:cfd-mr-ind-intersection}Difference in Accuracy between Males and Females for \textsc{CFD-MR} and \textsc{CFD-India}}
\caption{\label{tab:cfd-mr-ind-intersection}\textbf{Difference in highest accuracy and lowest accuracy between Males and Females for \textsc{CFD-MR} and \textsc{CFD-India}. Most results show significant disparity in prediction accuracy towards Males. AWS and Face++ report the largest disparities for all tasks on the Newsprint adversarial input for both datasets and Microsoft reports no disparity in Gender detection for \textsc{CFD-MR}.}}
\end{table*}

Here, we only discuss the disparities in accuracy between Males and Females in each of the datasets, for the sake of brevity. The results for \textsc{CFD-MR} are in Table \ref{tab:cfd-mr-gender} and for \textsc{CFD-India} in Table \ref{tab:cfd-india-gender}.

%\subsubsection{Disparity in \textsc{CFD-MR}}

\textbf{Observation.} From Table \ref{tab:cfd-mr-gender} we can see that Microsoft reports no disparity in accuracy for any of the inputs for the task of gender detection, whereas both AWS and Face++ report high disparties, specially for Newsprint filter. AWS reports $\approx 64\%$ against Males whereas Face++ reports $\approx 69\%$ against Females. The observations are similar for \textsc{CFD-India} (Table \ref{tab:cfd-india-gender}). Thus even ethnicities of other countries suffer from a similar bias as minority groups in USA.

For the task of age prediction, it can be seen that Microsoft is the most disparate FRS for \textsc{CFD-MR} (Table \ref{tab:cfd-mr-gender}) while AWS is for \textsc{CFD-India} (Table \ref{tab:cfd-india-gender}). 

\textbf{Key Takeaways.}
The key takeaways from the above observations are--
\begin{itemize}
	\item Both the extension datasets- \textsc{CFD-MR} and \textsc{CFD-India} experience disparity in accuracy between Males and Females. 
	\item Face++ is the most disparate FRS in \textsc{CFD-MR} while AWS is the most disparate in \textsc{CFD-India}.
	\item Newprint filter results in the most instances of disparity
\end{itemize}

%From Table , we can see that for the task of Gender detection, Microsoft reports no bias for any of the image sets, which can be correlated with $100\%$ accuracy reported from Figure \ref{Fig: MSFT-cfd-mr-accuracy}. On the contrary, we can see that both AWS and Face++ report significantly large biases for the Newsprint filter images. Infact, Face++ is unable to identify the gender of a single female. AWS performs exactly opposite and identifies females more than males with a bias of $-63.65\%$. 
%
%Similarly for the task of age prediction, it can be seen that Microsoft is able to reduce the bias whereas both AWS and Face++ report an increase of bias in Newsprint. Interestingly, both AWS and Microsoft report a lower bias for RGB filter for both the tasks.
%
%\textbf{Bias in \textsc{CFD-India}} Table \ref{tab:cfd-ind-intersection} shows the results of bias between the two genders for the task of gender and age prediction. Here again, Microsoft reports the lowest bias of $\approx 2\%$ for gender identification. AWS and Face++ perform similar as they did for \textsc{CFD-MR} with extremely high bias values of $-58.16\%$ and $62.9\%$ respectively. 
%
%For the task of age prediction, we can see that AWS has the highest bias of $\approx 23\%$ on RGB filter images and Face++ has the lowest-- $-9.23\%$. Microsoft reports a high bias for the Newsprint filter with males better than females by $17.48\%$.
%
%There results show that even for ethnicities that are not usually used for audit studies, large biases exist across gender for both gender and age predicition tasks.


% \subsection{Observations for \textsc{CFD-MR} and \textsc{CFD-India}}
% Along with \textsc{CFD}, we evaluated two other datasets- \textsc{CFD-MR} and \textsc{CFD-India} to study the bias that may be propagated for people belonging to ethnicities that are not commonly studied in the context of FRS.
% Here, we discuss the overall accuracy for the two datasets in a similar manner as above and also present a short discussion of the bias in accuracy for the two genders for both these datasets.

% \subsubsection{Prediction Accuracy for Adversarial Inputs}
% \if 0 
% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}{0.66\columnwidth}
% 		%\centering
% 		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/AWS_G_A_S_CFD_IND-new.pdf}
% 		% 		\vspace*{-4mm}
% 		\caption{Accuracy on AWS}
% 		\label{Fig: AWS-cfd-ind-accuracy}
% 	\end{subfigure}%
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\centering
% 		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/FPP_G_A_S_CFD_IND-new.pdf}
% 		%\vspace*{-3.5mm}
% 		\caption{Accuracy on Face++}
% 		\label{Fig: FPP-cfd-ind-accuracy}
% 	\end{subfigure}
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\centering
% 		\includegraphics[width= \textwidth, height=4.5cm, keepaspectratio]{plots/MSFT_G_A_S_CFD_IND-new.pdf}
% 		%\vspace*{-3.5mm}
% 		\caption{Accuracy on Microsoft}
% 		\label{Fig: MSFT-cfd-ind-accuracy}
% 	\end{subfigure}
	
% 	%\vspace*{-4mm}
% 	\caption{{\bf Performance on \textsc{CFD-India} for Original, RGB-Filter and Newsprint-filter inputs }}
% 	\label{fig:cfd-ind-accuracy}
% 	%\vspace{-4 mm}
% \end{figure*}
% \fi 
% We present the results for accuracy of prediction for the tasks of gender and age detection for \textsc{CFD-MR} in Figure \ref{fig:cfd-mr-accuracy} and for \textsc{CFD-India} in Figure \ref{fig:cfd-ind-accuracy}. 

% \textbf{Gender Detection.} For both the datasets, we see that all APIs have an accuracy of $> 90\%$ with Microsoft reporting an accuracy of $100\%$ for both the datasets. Here, Face++ is the weakest FRS with an accuracy of $\approx 90\%$ for \textsc{CFD-MR}(Figure \ref{Fig: FPP-cfd-mr-accuracy}) and $\approx 92\%$ for \textsc{CFD-India}(Figure \ref{Fig: FPP-cfd-ind-accuracy}). 
% For RGB-filtered images, the accuracy drop is minimal with Face++ infact reporting an increase in accuracy for \textsc{CFD-India} as can be seen in Figure \ref{Fig: FPP-cfd-ind-accuracy}. Thus similar to CFD-USA, these datasets also don't get impacted by RGB-filter.
% For Newsprint-filter we notice a significant drop in accuracy for both AWS and Face++ APIs, but almost no drop in accuracy for Microsoft. Face++ reports a drop in accuracy to $\approx 20.4\%$ in Figure \ref{Fig: FPP-cfd-mr-accuracy}. A similiar drop in accuracy is observed for both AWS and Face++ in \textsc{CFD-India} as well from Figures \ref{Fig: AWS-cfd-ind-accuracy} and \ref{Fig: FPP-cfd-ind-accuracy}.

% \textbf{Age Prediction.} Similar to \textsc{CFD}, Microsoft is the best performing API here and Face++ the worst, for both the datasets. The behaviour of the APIs for the different filters does not follow any pattern here, with Face++ reporting a lesser accuracy for RGB-filter than for Newsprint-filter (Figures \ref{Fig: FPP-cfd-mr-accuracy}, \ref{Fig: FPP-cfd-ind-accuracy}). AWS and Microsoft report alternating behaviour(ref. Figures \ref{Fig: AWS-cfd-mr-accuracy} and \ref{Fig: MSFT-cfd-mr-accuracy}, and Figures \ref{Fig: AWS-cfd-ind-accuracy} and \ref{Fig: MSFT-cfd-ind-accuracy}. The lowest accuracy is reported by Face++ for RGB-filter on \textsc{CFD-India} at $13.4\%$.

% Thus, we can see here that even with varied ethnicities, there is an impact on the accuracy of prediction for adversarial inputs.
% Here as well, Microsoft has the best accuracy on the adversarial images and Face++ has the worst.

% \begin{table*}[!ht]
% 	\centering
% 	\begin{subtable}{.4\linewidth}
% 	    \small
% 		\centering
% 		\begin{tabular}{c | c | c } 
% 			\hline
% 			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} \\
% 			\hline
% 			AWS/Original\rule{0pt}{2ex} & $3.23\%$ & $-10.04\%$ \\ 
% 			AWS/RGB\rule{0pt}{2ex} &  $-2.24\%$ & $7.69\%$ \\
% 			AWS/Newsprint\rule{0pt}{2ex} &  $\textbf{-63.65\%}$ &  $\textbf{-11.91\%}$ \\
% 			\cellcolor{red!20}Max. abs. inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{66.88\%(Newsprint)} & \cellcolor{red!20} \textbf{1.97\%(Newsprint)}\\
% 			\hline
% 			Face++/Original\rule{0pt}{2ex} & $12.90\%$ & $4.84\%$ \\ 
% 			Face++/RGB\rule{0pt}{2ex} & $-19.85\%$ & $8.93\%$ \\
% 			Face++/Newsprint\rule{0pt}{2ex} &  $\textbf{69.23\%}$ & $\textbf{29.03\%}$ \\
% 			\cellcolor{red!20}Max. abs. inc in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{56.33\%(Newsprint)} & \cellcolor{red!20} \textbf{24.19\%(Newsprint)}\\
% 			\hline
% 			Microsoft/Original\rule{0pt}{2ex} & $0\%$&  $\textbf{18.12\%}$ \\ 
% 			Microsoft/RGB\rule{0pt}{2ex} &  $0\%$ &  $17.49\%$ \\
% 			Microsoft/Newsprint\rule{0pt}{2ex} &  $0\%$ &  $-7.2\%$ \\
% 			\cellcolor{red!20}Max. abs. inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{$\phi$} & \cellcolor{red!20} \textbf{$\phi$}\\
% 			\hline
% 		\end{tabular}
% 	\caption{\textsc{CFD-MR}}\label{tab:cfd-mr-intersection}
% 	\end{subtable}%
	
% 	\begin{subtable}{.4\linewidth}
% 	    \small
% 		\centering
% 		\begin{tabular}{c | c | c } 
% 			\hline
% 			\textbf{Image}\rule{0pt}{2ex} & \textbf{Gender} & \textbf{Age} \\
% 			\hline
% 			AWS/Original\rule{0pt}{2ex} & $3.85\%$ & $15.77\%$ \\ 
% 			AWS/RGB\rule{0pt}{2ex} &  $7.69\%$ & $\textbf{23.08\%}$ \\
% 			AWS/Newsprint\rule{0pt}{2ex} &  $\textbf{-58.16\%}$ &  $-16.75\%$ \\
% 			\cellcolor{red!20}Max. abs inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{62.01\%(Newsprint)} & \cellcolor{red!20} \textbf{32.52\%(Newsprint)}\\			
% 			\hline
% 			Face++/Original\rule{0pt}{2ex} & $19.23\%$ & $4.36\%$ \\ 
% 			Face++/RGB\rule{0pt}{2ex} & $-0.30\%$ & $\textbf{-9.23\%}$ \\
% 			Face++/Newsprint\rule{0pt}{2ex} &  $\textbf{62.90\%}$ & $-1.07\%$ \\
% 			\cellcolor{red!20}Max. abs inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{43.67\%(Newsprint)} & \cellcolor{red!20} \textbf{13.59\%(RGB)}\\
% 			\hline
% 			Microsoft/Original\rule{0pt}{2ex} & $0\%$&  $-0.64\%$ \\ 
% 			Microsoft/RGB\rule{0pt}{2ex} &  $0\%$ &  $5.56\%$ \\
% 			Microsoft/Newsprint\rule{0pt}{2ex} &  $\textbf{1.92\%}$ & $\textbf{17.48\%}$ \\
% 			\cellcolor{red!20}Max. abs inc. in disparity\rule{0pt}{2ex} & \cellcolor{red!20} \textbf{1.92\%(Newsprint)} & \cellcolor{red!20} \textbf{18.12\%(Newsprint)}\\
% 			\hline
% 		\end{tabular}
% 		\caption{\textsc{CFD-India}}\label{tab:cfd-ind-intersection}
% 	\end{subtable}
% %\caption{\label{tab:cfd-mr-ind-intersection}Difference in Accuracy between Males and Females for \textsc{CFD-MR} and \textsc{CFD-India}}
% \caption{\label{tab:cfd-mr-ind-intersection}\textbf{Difference in highest accuracy and lowest accuracy between Males and Females for \textsc{CFD-MR} and \textsc{CFD-India}. Most results show significant disparity in prediction accuracy towards Males. AWS and Face++ report the largest disparities for all tasks on the Newsprint adversarial input for both datasets and Microsoft reports no disparity in Gender detection for \textsc{CFD-MR}.}}
% \end{table*}

% \subsubsection{Bias over Genders}
% Finally, we evaluate the change in bias between Males and Females due to the application of the adversarial filters. The results are presented in Table \ref{tab:cfd-mr-ind-intersection}. 


% \textbf{Bias in \textsc{CFD-MR}}
% From Table \ref{tab:cfd-mr-intersection}, we can see that for the task of Gender detection, Microsoft reports no bias for any of the image sets, which can be correlated with $100\%$ accuracy reported from Figure \ref{Fig: MSFT-cfd-mr-accuracy}. On the contrary, we can see that both AWS and Face++ report significantly large biases for the Newsprint filter images. Infact, Face++ is unable to identify the gender of a single female. AWS performs exactly opposite and identifies females more than males with a bias of $-63.65\%$. 

% Similarly for the task of age prediction, it can be seen that Microsoft is able to reduce the bias whereas both AWS and Face++ report an increase of bias in Newsprint. Interestingly, both AWS and Microsoft report a lower bias for RGB filter for both the tasks.

% \textbf{Bias in \textsc{CFD-India}} Table \ref{tab:cfd-ind-intersection} shows the results of bias between the two genders for the task of gender and age prediction. Here again, Microsoft reports the lowest bias of $\approx 2\%$ for gender identification. AWS and Face++ perform similar as they did for \textsc{CFD-MR} with extremely high bias values of $-58.16\%$ and $62.9\%$ respectively. 

% For the task of age prediction, we can see that AWS has the highest bias of $\approx 23\%$ on RGB filter images and Face++ has the lowest-- $-9.23\%$. Microsoft reports a high bias for the Newsprint filter with males better than females by $17.48\%$.

% There results show that even for ethnicities that are not usually used for audit studies, large biases exist across gender for both gender and age predicition tasks.

%================Commented by AD================
\if 0 
\begin{figure}
	\centering     %%% not \center
	\subfigure[AWS]{\label{fig2:a}\includegraphics[width=.5\textwidth,height=6cm,keepaspectratio]{plots/AWS_G_A_S_CLBST.pdf}}\\
	\subfigure[Face++]{\label{fig2:b}\includegraphics[width=.5\textwidth,height=6cm,keepaspectratio]{plots/FPP_G_A_S_CLBST.pdf}}\\
	\subfigure[Microsoft]{\label{fig2:c}\includegraphics[width=.5\textwidth,height=6cm,keepaspectratio]{plots/MSFT_G_A_S_CLBST.pdf}}
	\caption{Performance on \textsc{CelebSET}}\label{fig:celebset-accuracy}
\end{figure}
\fi 

\if 0 
\begin{figure}
	\centering     %%% not \center
	\subfigure[AWS]{\label{fig2:a}\includegraphics[width=.5\textwidth,height=6cm,keepaspectratio]{plots/AWS_G_A_CFD_USA.pdf}}\\
	\subfigure[Face++]{\label{fig2:b}\includegraphics[width=.5\textwidth,height=6cm,keepaspectratio]{plots/FPP_G_A_CFD_USA.pdf}}\\
	\subfigure[Microsoft]{\label{fig2:c}\includegraphics[width=.5\textwidth,height=6cm,keepaspectratio]{plots/MSFT_G_A_CFD_USA.pdf}}
	\caption{Performance on \textsc{CFD}}\label{fig:cfd-accuracy}
\end{figure}
\fi 

==> flow.tex <==
\if 0 
Introduction
	AI and its effect on life and livelihood
	Facial recognition system and its usage
	Prior audits on these systems
	Temporal and Emergent biases and need for continuous audit
	Need for adversarial audit
	Contribution - (+1 line obsv)

Background and related works
	Facial recognition systems: Microsoft, Amazon AWS, Face++
	Bias in facial recognition systems
	Adversarial auditing

Dataset for Auditing Facial Recognition Systems
	Datasets
		Celebset
		Chicago Face Dataset
	Adversarial Inputs
		Necessity
		Filters used

Experiment and observations
	On Celebset
		General audit
		Adversarial audit
	On CFD
		General audit
		Adversarial audit
	On CFD-MR and CFD-India
		General audit
		Adversarial audit

Conclusion
	Contribution
	Societal consequence and proposal for continuous audits
	Future work
\fi 

==> introduction-backup.tex <==
\section{Introduction}
\label{sec:intro}

Image recognition and analysis tasks have improved and diversified significantly over the past few years thanks to various deep learning techniques like CNNs. This has led to their use for numerous tasks like object and scene detection, facial analysis/re-identification/comparison, smile/emotion detection, etc. The accuracy of any deep learning task, including face detection, is highly dependent on the training data and on the relevant features. Publicly available datasets like LFW \cite{raji2021face} have given researchers and developers access to a large amount of data which has led to the proliferation of different architectures for solving these tasks. With the advent of cheap cloud-based services by vendors like Amazon AWS, Microsoft Azure and Google GCP the cost of deployment has also become minuscule and in turn has led to large-scale adoption by users. Such an unconstrained growth has come at the price of privacy, security and biased performance. 

Multiple past works like Propublica's study of \textsc{COMPAS}\footnote{https://bit.ly/3eGor3h} recidivism algorithm, Gender Shades \cite{buolamwini2018gender} and Bolukbasi et al.'s work \cite{bolukbasi2016man} have shown that AI-systems are biased and these biases are propagated from the real-world either because of the training data or how the algorithm is designed. This has resulted in unfair outcomes for members of particular communities. 

Although there have been attempts to formally define these biases \cite{mehrabi2019survey}, the domain is still fairly new, and thus requires an in-depth exploration.

It has been observed that commercial face detection software by vendors like IBM, Microsoft, Face++ and Amazon have an inherent bias when detecting faces of people belonging to non-white ethnicities or the female gender\cite{buolamwini2018gender, raji2020saving}. This can be attributed to either a biased training data or some inherent flaw in the detection algorithm which unfairly detects white faces with a higher accuracy. Understanding this problem is further impeded by the fact that these vendors do not provide open access to their models nor have they published model cards\cite{mitchell2019model} which can be used to get an idea about what the model entails. Thus, the only way to evaluate the bias in these software is to conduct black box audits. These audits attempt to determine the accuracy of the systems by providing input images of individuals belonging to different gender, age, and ethnic groups. 

Researchers in the AI community have performed multiple audit-based studies\cite{buolamwini2018gender,kyriakou2019,raji2019action,raji2020saving} of these commercial Facial Analysis Softwares(FAS) to determine the extent of bias in these systems on either standard face image datasets like the Chicago Face Database(\textsc{CFD}) \cite{ma2015chicago} or developed their own benchmark datasets like \textsc{PPB} \cite{buolamwini2018gender} and \textsc{CelebSET}\cite{raji2020saving}. These audits show that the commercial systems continue to propagate biased outcomes over time, exhibiting both \textit{temporal bias} and \textit{emergent bias} \cite{mehrabi2019survey}. 

Based on the above observations and our own experiments, it is evident that these biases continue to exist and therefore there is an urgent need to establish non-governmental international bodies that not just formally define what constitutes bias in this scenario, but also conduct regular audits of these systems so that the users are aware of the side-effects of their applications.

On the other side of the coin, there have been a lot of studies on adversarial attacks against Facial Recognition Systems \cite{vakhshiteh2020adversarial}. These attacks could range from very simple to extremely complex and have been successful in fooling both open-source architectures and commercial products. Even simpler tools like social media apps(Instagram, Snapchat, etc.) provide users with various filters to edit images. Thus, with such easy access to image perturbation techniques, bad actors may be able to use these filtered images to mis-train or misclassify input images. All these techniques perturb input images and cause misclassification by the FAS, but they don't attempt to study the biases in the output due to these perturbations. 

In this study we attempt to answer the following question-- \textit{Does the bias in accuracy for Facial Analysis Software change for adversarial input images?} As per our knowledge, this is the first such study that attempts to formally evaluate biases in commercial face detection softwares for adversarial inputs. 

The rest of the paper is organized as follows- Section \ref{sec:rel-work} discusses the related literature in this field, Section \ref{sec:dataset-perturb} presents the details of the input datasets, the perturbation techniques used and the FAS evaluated as part of this audit, Section \ref{sec:experiments} presents the results on accuracy and bias across the different groups. We conclude our argument in Section \ref{sec:conclusion}.
